Understanding Cross-modal Interactions in V&L Models that Generate Scene Descriptions

Image captioning models tend to describe images in an object-centric way, emphasising visible objects. But image descriptions can also abstract away from objects and describe the type of scene depicted. In this paper, we explore the potential of a state-of-the-art Vision and Language model, VinVL, to caption images at the scene level using (1) a novel dataset which pairs images with both object-centric and scene descriptions. Through (2) an in-depth analysis of the effect of the fine-tuning, we show (3) that a small amount of curated data suffices to generate scene descriptions without losing the capability to identify object-level concepts in the scene; the model acquires a more holistic view of the image compared to when object-centric descriptions are generated. We discuss the parallels between these results and insights from computational and cognitive science research on scene perception.

==> attention.tex <==
\section{Analysing  Multimodal Interactions }
% It is known that large language models can easily adapt in few-shots to a new task \cite{brown2020language} and VinVL confirm this expectation.
In our investigation, we wonder about changes in the model's inner dynamics during fine-tuning. We expect to find differences in the multimodal interplay involving the visual and the textual modality. Therefore, we will investigate on aspects involving key internal mechanisms, like self-attention and inner representations of the model, trying to shed light on the way VinVL uses object information to generate descriptions. 

% We are interested in multimodal interplay involving vision and text. However, the interactions with object tags are also interesting because, as highlighted by \cite{li2020oscar} they can be considered both visual and textual input at the same time they may provide a possible bridge between the two modalities.

\subsection{Self-attention}
\label{sec:attention}
Little is known about the exact mechanisms allowing by BERT-based models to achieve outstanding performance.
However, the self-attention plays often a central role in the model's interpretation and therefore is commonly used to address this issue \cite{kovaleva2019revealing, clark2019does, vishwamitra2020analyzing}, even though, its interpretation is not always clearly understood. 

We select 100 random samples of the test-set and we extract the attention matrices before and after fine-tuning on scene descriptions. We aggregate the attention matrix at each layer by taking the maximum value across all the heads, as we found this method useful to visualize the interactions between the input modalities.

To analyse multimodal interaction, we focus on the self-attention patterns visible in the first layer, as they are directly connected to the inputs and do not depend on higher-level interactions which might obscure the fundamental changes in attention across the three modalities (visual features, labels and text) in VinVL.
%make harder any kind of interpretation. 
At higher layers, we observe  a unique self-attention pattern focusing on the [SEP] token; we return to this phenomenon below (\ref{para:special_token}).

% models' self-attention matrices, we observe a broader attention at lower layers which becomes more focused at higher layers, as observed by \cite{scialom2020bert}. The lower layers are the most suitable for observing inputs interaction as the attention still preserve semantic information, that is gradually lost in the top layers. 

\paragraph{Scenes as a whole}
As shown in Figure~\ref{fig:attention-comparison}, the self-attention of the pre-trained model is sharper and results accumulated on specific inputs, with very high peaks for some inputs and almost none for others. After fine-tuning, the self-attention is evenly distributed over the inputs. This suggest that when generating scenes the model leverages a wider range of visual features.

We perform a quantitative analysis of the self-attention. We select those sub-blocks of the self-attention matrix involving visual regions and object labels and we compute the standard deviation of the attention weights in these sub-blocks for each sample. The result is shown in Figure~\ref{fig:att-std}. By looking at the distributions of the attention mass and the standard deviations in the self-attention sub-blocks before and after fine-tunining, it is evident that the fine-tuned model has a lower standard deviation than the pre-trained model. In other words, fine-tuning on scene descriptions results in the model distributing attention mass more evenly across the inputs. 
%AG: Added the below
We take this as evidence that in the process of generating scene descriptions, the fine-tuned model requires a more holistic view of the input image, in contrast to the highly object-centred deployment of attentional resources evident in the pre-trained model.
% eaning that after finetuning the attention is more evenly distributed. In other words, this stems the hypothesis that after the exposure to scene descriptions the model has acquired  a more holistic view of the picture.

% confirm that the finetuned model's attention has indeed a lower standard deviation than the pretrained model, meaning that after finetuning the model acquired a more holistic view of the picture.

% scene-object relationships, RBO, etc.
\paragraph{Scene-Object relationship}
VinVL re-settles its self-attention to a wider range of visual features when generating scenes, however this does not imply that it is not focusing more on some objects then others, in fact we expect the model to be attending more to some objects useful to generate the scene. 


% Although, the attention is more diffused across the visual features, we expect the model to be focusing more on relevant objects for the scene.
In order to study the relationship between objects and scenes we proceed as follows:
\begin{enumerate}
    \item $ \forall \; s \; in \; S$ we collect $ O_M^s = [ o_1^s, o_2^s, ..., o_n^s ] $ where $S$ is the set of the most frequent scenes in the sample and $O_M^s$ is the ranked list of the most attended objects by the model $M$ when generating scene $s$. 
    \item Similarly $ \forall \; s \; in \; S$ we collect $ O_D^s = [ o_1^s, o_2^s, ..., o_n^s ] $ where $S$ is the same set of the most frequent scenes in the sample and $O_D^s$ is the ranked list of the most frequent objects for the scene $s$ in the dataset $D$. 
\end{enumerate}
% We compute the most common objects of the most common scenes in our dataset. We assign to each image in our 100 samples the corresponding scene with the list of the most common objects in the scene.
% From the attention matrices we extract the most attended objects by the model when generating the scene.
We then have two ranked lists of objects, the most attended objects by the model when generating the scenes  ($O_M^s$) and the most frequent objects for the scene in the dataset  ($O_D^s$).


We measure the overlap of these two lists by computing the Intersection over Union (IoU). Moreover, since we are also interested to the rank of the object in the list, we measure the Rank Biased Overlap (RBO)\footnote{\href{}{https://github.com/changyaochen/rbo}}\cite{webber2010similarity} between the two lists. The RBO is a metric used to compute the similarity of two ranked lists and it follows the following formulation:
\begin{equation}
    RBO(S, T, p) = (1-p)\sum p^{d-1}A_d
\end{equation}

where $d$ is the depth of the ranking being examined, $A_d$ is the agreement between $S$ and $T$ given by the proportion of the size of the overlap up to $d$, $p$ determine the contribution of the top $d$ ranks to the final RBO measure, we use the standard value  $p=1$.

\input{tables/rbo}

We compute RBO and IoU for the top 3, 5 and 7 objects of the lists and we report the results in Table~\ref{rbo}. Both metrics range between 0 and 1 where, 0 means no overlap (for IoU) or zero similarity (for RBO) and 1 means identical. Interestingly, we observe that the two metrics correlate strongly ($r(19)=.81, p<.001$) meaning that the model attends to the most common objects in the extend to which they are likely to be present in the scene when generating scene descriptions. 
% Moreover, we observe high scores for scenes like \textit{station, road, resort, sea}, namely for scenes easy to distinguish by looking at specific objects, whereas for scenes like \textit{room, house, restaurant} we observe lower scores, as they contain a wider variety of objects, that makes harder finding distinctive objects
Moreover, we observe high scores for scenes where frequent objects are more diagnostic of their environment like \textit{station, road, resort, sea}, whereas for scenes like \textit{room, house, restaurant} we observe lower scores, as they contain a wider variety of objects with lower semantic impact.

%VinVL leverages the assumption that many objects detected by the visual backbone are mentioned in the caption and by means of the object tags it provides anchor points that ease the grounding of objects between the two modalities, however by finetuninig with scene descriptions we brake this assumption. 


% not sure if we want to keep this section
\paragraph{Special tokens}
\label{para:special_token}
At higher layers the the attention gather around  the special token [SEP] used to separate the \textit{text + object tags} from the \textit{visual} input. A similar behaviour has been observed analysing BERT's attention performed by \cite{clark2019does}. %They argue that the [SEP] is used as a sort of no-op by the mode. We tent to be skeptical about this interpretation as this phenomenon is present only on one of the two [SEP] tokens of the input. 
We note that [SEP] token gathering all the attention never changes position in the input because of the padding,  therefore we tend to interpret it as a sort of pivot among the inputs

% TODO fix the size 
% TODO: Change this to use two subfigures with their own subcaptions
% See: https://www.overleaf.com/learn/latex/How_to_Write_a_Thesis_in_LaTeX_(Part_3)%3A_Figures%2C_Subfigures_and_Tables
\begin{figure*}[!t]
    \centering
     \includegraphics[scale=0.27]{imgs/att_comparison_ft_pre_highlighted.png}
    \caption{On the Left the attention matrix of the pre-trained model, on the Right the attention of the model fine-tuned on scene descriptions, highlighted the sub-block of the matrices involving visual information. Both the matrices refer to the sample sample}
    \label{fig:attention-comparison}
\end{figure*}



==> scratch.tex <==
This perspective continues to dominate current research, which relies on pretrained, transformer-based \vl models \cite[e.g.][]{li2020oscar,zhang2021vinvl,Hu2021}. 
The object-centric nature of the task is reinforced by two factors. First, the visual backbone used by the majority of \vl models to extract visual features is typically pretrained on an object labelling task, such as ImageNet \cite{Deng2009,Russakovsky2015}. Second, datasets used for both pretraining and testing tend to pair images with captions which explicitly mention at least some of the objects in a scene \cite[e.g.][]{young-etal-2014-image,Chen2015,pont2020connecting,Gurari2019VizWizPrivAD,Sharma2018}. In the same spirit, the recently introduced \itt{nocaps} benchmark \cite{agrawal2019nocaps} is designed to test captioning models' ability to generalise to novel objects.

The object-centric nature of the captioning task has a clear rationale. After all a successful description of a picture would be expected to make reference to its contents. Nevertheless, 




